WCDT: Systematic WCET Optimization for Decision Tree Implementations

Machine-learning models are increasingly deployed on resource-constrained embedded systems with strict timing constraints. In such scenarios, the worst-case execution time (WCET) of the models is required to ensure safe operation. Specifically, decision trees are a prominent class of machine-learning models and the main building blocks of tree-based ensemble models (e.g., random forests), which are commonly employed in resource-constrained embedded systems. In this paper, we develop a systematic approach for WCET optimization of decision tree implementations. To this end, we introduce a linear surrogate model that estimates the execution time of individual paths through a decision tree based on the path's length and the number of taken branches. We provide an optimization algorithm that constructively builds a WCET-optimal implementation of a given decision tree with respect to this surrogate model. We experimentally evaluate both the surrogate model and the WCET-optimization algorithm. The evaluation shows that the optimization algorithm improves analytically determined WCET by up to $17\%$ compared to an unoptimized implementation.

==> sections/WCETmodel.tex <==
\label{sec:WCETmodel}

\rev{1}{I inferred from the description of the SiC architecture from section 6 that SiC has no branch predictor, or a very simple one. Is my interpretation correct? More details on that aspect would be very welcome.}

In this section, we detail the hardware model underlying the WCET analysis employed in this paper.
Specifically, the following model is used in our empirical evaluation.

We assume a single-core strictly-in-order (SIC) processor~\cite{Hahn2015,SIC}, which enforces that all hardware resources are used by instructions in the program order.
This means, that all instructions enter end exit every pipeline stage in the same order as they occur in the program execution, which allows a significantly more efficient pipeline analysis, as timing anomalies are provably avoided.
The SIC processor has a five-stage pipeline consisting of the following stages: instruction fetch, instruction decode, execute, memory access, and write back.
The memory hierarchy consists of separate single-level instruction and data caches and a unified background memory.




Both caches share a bus to access the background memory.
Memory accesses are
the result of cache misses due to the instruction fetch and the memory stage.
To enforce strictly in-order execution, data-cache misses are prioritized over instruction-cache misses.
All memory levels have a known constant latency.
Furthermore, the caches employ LRU replacement, which ensures predictable behavior~\cite{Reineke07}, even if the initial cache states are unknown.


Our method specifically focuses on the behavior of conditional branching and the corresponding effect on the WCET.\@
Conditional branch instructions have a single-cycle latency in case they are not taken.
Yet, if a branch is taken, the pipeline is flushed and the branch target is fetched, resulting in a longer delay.
In addition to the immediate cost of flushing the pipeline upon a taken branch, the branch target is usually not in the same cache line as the branch instruction, which may cause an additional cache miss compared to the untaken branch.


We use LLVMTA~\cite{llvmta} to perform static code analysis for estimating the WCET\@.
LLVMTA is a timing analysis framework that utilizes information handed down from LLVM during the analysis process. It uses a simple background memory model, where a cache miss is assumed to have a constant penalty of 100 cycles.


%%% Local Variables:
%%% TeX-master: "../conference_101719"
%%% End:

